Frobenius Additive Fast Fourier Transform

In ISSAC 2017, van der Hoeven and Larrieu showed that evaluating a polynomial P in GF(q)[x] of degree <n at all n-th roots of unity in GF($q^d$) can essentially be computed d-time faster than evaluating Q in GF($q^d$)[x] at all these roots, assuming GF($q^d$) contains a primitive n-th root of unity. Termed the Frobenius FFT, this discovery has a profound impact on polynomial multiplication, especially for multiplying binary polynomials, which finds ample application in coding theory and cryptography. In this paper, we show that the theory of Frobenius FFT beautifully generalizes to a class of additive FFT developed by Cantor and Gao-Mateer. Furthermore, we demonstrate the power of Frobenius additive FFT for q=2: to multiply two binary polynomials whose product is of degree <256, the new technique requires only 29,005 bit operations, while the best result previously reported was 33,397. To the best of our knowledge, this is the first time that FFT-based multiplication outperforms Karatsuba and the like at such a low degree in terms of bit-operation count.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

PDF = main.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $< -synctex=1; done


%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

affft.pdf : body.tex



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi $(PDF)

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf


==> benchmark.tex <==
\section{Implementation Details}
\subsection{Basis conversion}
The choice of the algorithm. Consider the cache efficiency.
\subsection{Frobenius Encoding and Decoding}
Matrix vector product over $\GF{2}$. transpose
\subsection{Finite field arithmetic}
PCLMULQDQ
\subsection{Butterfly network}
cache efficiency?
\section{Timings}
State the testing environment. Turn off turbo? 
State the libraries we test. cite recent development

Benchmark on Intel Haswell architecture Table~\ref{tab:ranger}


Benchmark on Intel Skylake architecture Table~\ref{tab:angel1}

\begin{table*}
\begin{center}
%\small
\begin{threeparttable}
\caption{Products in degree $< d$ in $\GF{2}[x]$ on Intel Haswell Xeon E3-1245 v3 @ 3.40GHz ($10^{-3}$ sec.)
%with AVX2 instruction set, in milliseconds.
}
\label{tab:ranger}
\begin{tabular}{l  r  r  r r  r  r  r  r  r  }
\toprule
   $\log_2 d/64$ & 15 & 16  & 17 &  18 & 19 & 20 & 21 & 22 & 23   \\ 
\midrule

This work      & 6 & 14 & 29 & 61 & 131 & 282 & 597 & 1270 & 2666 \\
FDFT \cite{vanderhoeven:hal-01579863} \tnote{c} & 6 &  15 &  32  &  72   & 165   & 311   &  724  & 1280 & 3397 \\  
AFFT\cite{DBLP:journals/corr/abs-1708-09746} with $\TGF{2^{256}}$               &  9 & 19 & 40 &  90 & 212 & 463 & 982 & 2050 & 4299  \\
$\GF{2^{60}}$ \cite{DBLP:conf/issac/HarveyHL16} \tnote{b} & 14 &  29 &  64  &  148   & 279   & 668   &  1160  & 3142 & 7040 \\  
%This work, $\TGF{2^{128}}$          & 11 & 22 & 48 & 104 & 243 & 527 & 1105 & 2302 & 4812  \\  \hline 
%This work, $\GF{2^{128}}$      & 12 & 26 & 55 & 119 & 261 & 554 & 1181 & 2491 & 5282 \\  \hline \hline
\texttt{gf2x} \cite{gf2x} \tnote{a}  & 12 & 26 & 59 & 123 & 285 & 586 & 1371 & 3653 & 7364  \\ 
\bottomrule
\hline
\end{tabular}
\begin{tablenotes}
  \small
%  \item [a] Evaluation points in Cantor basis.
  \item [a] Version 1.2.  Available from \url{http://gf2x.gforge.inria.fr/}
  \item [b] SVN r10663. Available from \url{svn://scm.gforge.inria.fr/svn/mmx}
  \item [c] SVN r10681. Available from \url{svn://scm.gforge.inria.fr/svn/mmx}
\end{tablenotes}
\end{threeparttable}
\end{center}
\end{table*}

\begin{table*}
\begin{center}
%\small
\begin{threeparttable}
\caption{Products in degree $< d$ in $\GF{2}[x]$ on Intel Skylake Xeon E3-1275 v5 @ 3.60GHz ($10^{-3}$ sec.)
%with AVX2 instruction set, in milliseconds.
}
\label{tab:angel1}
\begin{tabular}{l  r  r  r r  r  r  r  r  r  }
\toprule
   $\log_2 d/64$ & 15 & 16  & 17 &  18 & 19 & 20 & 21 & 22 & 23   \\ 
\midrule
This work, $\GF{2^{128}}$  &  4 & 9 & 20 &  41 & 88 & 192 & 418 & 889 & 1865 \\
FDFT \cite{vanderhoeven:hal-01579863} \tnote{c} & 4 &  11 &  24  &  56   & 127   & 239   &  574  & 958 & 2465 \\ 
ADFT\cite{DBLP:journals/corr/abs-1708-09746} with $\TGF{2^{256}}$          &  8 & 16 & 34 &  74 & 175 & 382 & 817 & 1734 & 3666  \\ 
$\GF{2^{60}}$\cite{DBLP:conf/issac/HarveyHL16}\tnote{b}  & 10 &  22 &  51  &  116   & 217   & 533   &  885  & 2286 & 5301 \\ 
\texttt{gf2x} \tnote{a} \cite{gf2x} & 11 & 23 & 51 & 111 & 250 & 507 & 1182 & 2614 & 6195  \\ 

\bottomrule
\hline
\end{tabular}
\begin{tablenotes}
  \small
%  \item [a] Evaluation points in Cantor basis.
  \item [a] Version 1.2.  Available from \url{http://gf2x.gforge.inria.fr/}
  \item [b] SVN r10663. Available from \url{svn://scm.gforge.inria.fr/svn/mmx}
  \item [c] SVN r10681. Available from \url{svn://scm.gforge.inria.fr/svn/mmx}
\end{tablenotes}
\end{threeparttable}
\end{center}
\end{table*}
\section{Conclusions}
%\end{document}  % This is where a 'short' article might terminate

%\begin{acks}
%  The authors would also like to thank the anonymous referees for
%  their valuable comments and helpful suggestions. 
%\end{acks}

